Stabilized finite element method for incompressible solid dynamics using an updated Lagrangian formulation

This paper proposes a novel way to solve transient linear, and non-linear solid dynamics for compressible, nearly incompressible, and incompressible material in the updated Lagrangian framework for tetrahedral unstructured finite elements. It consists of a mixed formulation in both displacement and pressure, where the momentum equation of the continuum is complemented with a pressure equation that handles incompresibility inherently. It is obtained through the deviatoric and volumetric split of the stress, that enables us to solve the problem in the incompressible limit. The Varitaional Multi-Scale method (VMS) is developed based on the orthogonal decomposition of the variables, which damps out spurious pressure fields for piece wise linear tetrahedral elements. Various numerical examples are presented to assess the robustness, accuracy and capabilities of our scheme in bending dominated problems, and for complex geometries.

==> fic.tex <==
%-------------------------------------------------------------------------------
% @collection	Multilevel methods
% @description 
% @version		1
% @author		Aurélien Larcher <aurelien.larcher@gmail.com>
%-------------------------------------------------------------------------------
% @category		Flux Interface Correction
%---------------------------------------
\newcommand{\w}{\omega}
% *c : coarse , *f: fine
\newcommand{\iI}{\bar\imath}% 1er indice local ex: faces
\newcommand{\jJ}{\bar\jmath}% 2e indice local ex: maille
\newcommand{\Kj}{K^{\jJ}}% maille raffinée
%%%%%% Set of Cells / Cells
\newcommand{\setC}{\mathcal{K}}% ensemble de volumes de controle
%\newcommand{\mesh}{{\cal M}}
\newcommand{\compmesh}{\underline{\disc}}
\newcommand{\Csetc}[1]{\mathcal{A}_{#1}}% ens. des volumes grossiers dans \domf
\newcommand{\Csetf}[1]{\mathcal{K}_{#1}}% ens. des volumes fins dans \domc
\newcommand{\Cneigh}[1]{\mathcal{N}(#1)}% ens. des voisins de K
\def\PSperp{\psline[linewidth=0.2pt](-0.15,0)(-0.15,0.15)(0,0.15)}
%%%%%% Set of Facets / Facets
\newcommand{\edgesimm}{\edges_{{\rm imm}}}% faces interface immergée
\newcommand{\Fkl}{K \vert L}% face K|L
\newcommand{\Fc}{\edge^{\iI}}% face grossière notation locale
\newcommand{\Ff}{\edge^{\iI,\jJ}}% face fine notation locale
\newcommand{\yF}{y_\edge}% barycentre face grossière
\newcommand{\yFc}{\yF^{\iI}}% barycentre face grossière
\newcommand{\yFf}{\yF^{\iI,\jJ}}% barycentre face fine
%%%%%% Operateurs
\newcommand{\oRdef}{\mathbf{R}^{l}_{l+1}}% opérateur de restriction
\newcommand{\oR}[2]{(\oRdef #1)_{#2}}% restriction appliquée à #1 en #2
\newcommand{\oPvdef}{\mathbf{P}}% op. de prolongement volumique
\newcommand{\oPv}[2]{(\oPvdef_{l}^{l+1} #1)_{#2}}% prolongement vol. de #1 en #2
\newcommand{\oPsdef}{\mathbf{\hat P}^{l+1}_{l}}% op. de prolongement surfacique
\newcommand{\oPs}[2]{(\opsdef #1)_{#2}}% prolongement de #1 en #2
\newcommand{\oRfdef}{\mathbf{\hat R}^{l}_{l+1}}% opérateur de restriction
\newcommand{\oRf}[2]{(\oRfdef #1)_{#2}}% restriction appliquée à #1 en #2
%%%%%% Espaces belonging to L^2(\Omega)
\newcommand{\xHc}{{\xHdisc^l}}% esp. des fct. VF sur maillage grossier
\newcommand{\xHf}{{\xHdisc^{l+1}}}% esp des fct. VF sur maillage fin
\newcommand{\xHcomp}{{\rm H}_{\compmesh}}% esp des fct. VF sur maillage fin
\newcommand{\xVc}{\mathcal{V}_l}% espace des appli. lin. de space(\domc) -> \xHc
\newcommand{\xVf}{\mathcal{V}_{l+1}}% espace des appli. lin. de space(\domf) -> \xHf


==> fvm.tex <==
%-------------------------------------------------------------------------------
% @collection	Finite Volume Method
% @description
% @version		1
% @author		Aurélien Larcher <aurelien.larcher@gmail.com>
%-------------------------------------------------------------------------------
% @subcategory	Fluxes
% @macro fluxK		outward flux from K across edge
\newcommand{\fluxK}{F_{\edge,K}}
% @macro fluxL  	outward flux from L across edge
\newcommand{\fluxL}{F_{\edge,L}}
% @macro fluxd
\newcommand{\fluxd}{F_{\edged,\edge}}
% @macro vs			outward velocity from K across edge
\newcommand{\vs}{\mathrm{v}_{K,\edge}}
% @macro vsp		positive part of the outward velocity from K across edge
\newcommand{\vsp}{\mathrm{v}_{\edge,K}^+}
% @macro vsm		negative part of the outward velocity from K across edge
\newcommand{\vsm}{\mathrm{v}_{\edge,K}^-}
% @macro vspd
\newcommand{\vspd}{\mathrm{v}_{\edged,\edge}^+}
% @macro vsmd
\newcommand{\vsmd}{\mathrm{v}_{\edged,\edge}^-}
%-------------------------------------------------------------------------------
% @category		Discrete Operators
% @macro Graddisc	discrete gradient
\newcommand{\Graddisc}{\mathop{\boldsymbol\nabla_\discd}}
% @macro Divdisc 	discrete divergence
\newcommand{\Divdisc}{\mathop{\boldsymbol\nabla_\discd\cdot}}
% @macro Lapdisc	discrete Laplace operator
\newcommand{\Lapdisc}{\mathop{\boldsymbol\Delta_\discd}}
% @macro DivGdisc	discrete 'Div(#1 Grad)' operator
\newcommand{\DivGdisc}[1]{\mathop{\boldsymbol\Delta_{\discd,#1}}}
% @macro GradK		restriction of the discrete gradient on K
\newcommand{\GradK}[1]{\mathop{\left[\Graddisc(#1)\right]_K}}
% @macro DivK		restriction of the discrete divergence on K
\newcommand{\DivK}[1]{\mathop{\left[\Divdisc(#1)\right]_K}}
% @macro LapK		restriction of the discrete Laplace operator on K
\newcommand{\LapK}[1]{\mathop{\left[\Lapdisc(#1)\right]_K}}
% @macro dtphi		discrete time derivative of the test function
\newcommand{\dtphi}{\partial_{t,\discd}(\varphi)}
% @macro dtu		discrete time derivative of u
\newcommand{\dtu}{\partial_{t,\discd}(u)}
% @macro dedge		variable of integration on edge
\newcommand{\dedge}{\, {\rm d} \gamma}
% @macro dtD		discrete derivative
\newcommand{\dtD}{\partial_{t,\discd}}
%-------------------------------------------------------------------------------
% @category		Discrete Spaces
% @macro xHdisc		finite volume H^1_0 space
\newcommand{\xHdisc}{{\rm H}_{\mesh}}
% @macro xHdiscb	finite volume
\newcommand{\xHdiscb}{\bar {\rm H}_{\mesh}}
% @macro xHdiscd	finite volume H^1_0 space
\newcommand{\xHdiscd}{{\rm H}_{\discd}}
% @macro xHdiscdb	finite volume H^1_0 space
\newcommand{\xHdiscdb}{\bar {\rm H}_{\discd}}
% @macro xHdisct	finite volume H^1_0 space
\newcommand{\xHdisct}{{\rm H}_{\disct}}
% @macro xHdiscm	finite volume H^1_0 space indexed by mesh
\newcommand{\xHdiscm}{\xHdisc^\m}
%-------------------------------------------------------------------------------
% @category		Discrete Norms and Seminorms
% @macro normVF		finite volume H^1 norm
\newcommand{\normVF}[1]{\norm{#1}_{1,\mesh}}
% @macro normVFn	finite volume W(1,q) norm
\newcommand{\normVFn}[2]{ \norm{#2}_{ 1,{#1},{\mesh} } }
% @macro snormVF	finite volume H^1 seminorm
\newcommand{\snormVF}[1]{\snorm{#1}_{1,\mesh}}
% @macro snormVFn	finite volume W(1,q) seminorm
\newcommand{\snormVFn}[2]{\snorm{#2}_{1,#1,\mesh}}
% @macro normVFmn	finite volume W(-1,n) norm
\newcommand{\normVFmn}[2]{|\hspace{-.1em}|#2|\hspace{-.1em}|_{-1,#1,\mesh}}


==> listofnotations.tex <==
\def\addnotation#1#2#3{\noindent$#1$\hfill \parbox{12cm}{#2 \dotfill}\\}
% \addnotation \alpha: {some variable that means something to me}{alpha}
%where : \addnotation    a TeX command you need to have 
%        \alpha:     the LaTeX code for the symbol. You don't have to add $...$ around math stuff. 
%                    Non-math symbols? Try it out. Be sure to add a trailing colon : to separate the entries. 
%        {some variable that means something to me}   the description of the variable, enclosed in curly brackets {} 
%        {alpha}     a label that you'll use to tag the first occurrence of the symbol. See the example source .tex file below. 
\def\newnotation#1{\label{#1}}
\def\listofnotations{\input symbols.tex}
\def\notations{\newpage\section{Notations}\markboth{List of Notations \hfill}{List of Notations \hfill}\listofnotations}
\def\NOMnew{\begin{center}\begin{tabular*}{16cm}{|ll@{\extracolsep{\fill}}c|}}
\def\NOMend{\end{tabular*}\end{center}}


==> mathenv.tex <==
%--- NEWTHEOREM AND ENVIRONMENTS------------------------------------------------
% passage des environments en anglais
%-------------------
\theoremstyle{plain}
%-------------------
\newtheorem{thrm}{Theorem}[section]
\newtheorem{lmm}[thrm]{Lemma}
\newtheorem{crllr}[thrm]{Corollary}
\newtheorem{prpstn}[thrm]{Proposition}
\newtheorem{crtrn}[thrm]{Criterion}
\newtheorem{lgrthm}[thrm]{Algorithm}
%------------------------
\theoremstyle{definition}
%------------------------
\newtheorem{dfntn}[thrm]{Definition}
\newtheorem{cnjctr}[thrm]{Conjecture}
\newtheorem{xmpl}[thrm]{Example}
\newtheorem{prblm}[thrm]{Problem}
\newtheorem{rmrk}[thrm]{Remark}
\newtheorem{nt}[thrm]{Note}
\newtheorem{clm}[thrm]{Claim}
\newtheorem{smmr}[thrm]{Summary}
%\newtheorem{cs}[thrm]{Case}
\newtheorem{bsrvtn}[thrm]{Observation}
\newtheorem{hypth}[thrm]{Assumption}
\newtheorem{xrcs}[thrm]{Exercise}
\newtheorem{sltn}[thrm]{Solution}

\theoremstyle{plain}
%------------------------------------------------------------------------------
\newenvironment{acknowledgement}{\par\addvspace{17pt}\small\rmfamily\noindent}{\par\addvspace{6pt}}
%------------------------------------------------------------------------------
%
\def\xProof{
  \normalfont
  \medskip
  {\noindent\itshape Proof.\hspace*{6pt}\ignorespaces}}
%
\endinput

%------------------------------------------------------------------------------


==> navierstokes.tex <==
%-------------------------------------------------------------------------------
% Navier-Sokes

\newcommand{\uu}{{\boldsymbol u}}
\newcommand{\uum}{\bar\uu}
\newcommand{\uup}{\tilde\uu}
\newcommand{\vv}{{\boldsymbol v}}
\newcommand{\ww}{{\boldsymbol w}}
\newcommand{\uuc}{\uu^\dagger}
\newcommand{\uucm}{\tilde\uu}

%-------------------------------------------------------------------------------
% Stokes
% Vector-valued divergence-free Sobolev a.k.a velocity
% version jean-claude :
\newcommand{\xVd}{{\bfV}}
\newcommand{\xVddisc}{{\xVd}_h}
\newcommand{\xVddiscm}{{\xVddisc}^{(m)}}
% Pressure
\newcommand{\xX}{{\rm X}}
\newcommand{\xXdisc}{{\xX}_{h}}
\newcommand{\xXdiscm}{{\xXdisc}^{(m)}}



==> notations.tex <==
\addnotation{\grad}{gradient}{grad}
\addnotation{\lapl}{laplacian}{lapl}
\addnotation{\dens}{density}{dens}
\addnotation{\cond}{conductivity}{cond}
\addnotation{\visc}{dynamic viscosity ($Pa.s$)}{visc}
\addnotation{\kvisc}{kinematic viscosity ($m^2/s$)}{kvisc}
\addnotation{\tension}{surface tension}{tension}
\addnotation{\Tt}{surface tension}{Tt}
\addnotation{\Ttm}{constante}{Ttm}
\addnotation{\cp}{chaleur massique}{cp}
\addnotation{\fric}{coefficient de friction}{fric}
\addnotation{\xCzero}{space of continuous functions}{xCzero}
\addnotation{\xCinfty}{space of smooth functions}{xCinfty}
\addnotation{\xHone}{sobolev space}{xHone}
\addnotation{\xLtwo}{space of finite energy functions}{xLtwo}


==> turbulence.tex <==
%-------------------------------------------------------------------------------
% Turbulence Models
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
% Averaging Operators
\newcommand{\avrg}[1]{{\overline{#1}}}

%-------------------------------------------------------------------------------
% k-epsilon
\newcommand{\kk}{k}
\newcommand{\eps}{\varepsilon}
\newcommand{\keps}{\kk-\eps}
\newcommand{\rng}{\mathrm{RNG}}
\newcommand{\kepsrng}{\keps\ \rng}

% constants
\newcommand{\Cmu}{C_\mu}
\newcommand{\Ckp}{C_{k1p}}
\newcommand{\Ckg}{C_{k1g}}
\newcommand{\Cke}{C_{k2}}
\newcommand{\Ceps}[1]{C_{\varepsilon#1}}
\newcommand{\Cek}{C_{\eps 1}}
\newcommand{\Cee}{C_{\eps 2}}
\newcommand{\Cerng}{C_{\eps 3}}
\newcommand{\Crng}{C_{\rm{rng}}}
\newcommand{\Cep}{C_{\eps 1}}
\newcommand{\Cepz}{C^z_{\eps 1}}
\newcommand{\Cega}{C_{\eps 1ga}}
\newcommand{\Cegb}{C_{\eps 1gb}}
\newcommand{\Ceta}{C_{\eta}}
% source terms
\newcommand{\sG}{\mathbf{G}}
\newcommand{\sP}{\mathbf{P}}
\newcommand{\sS}{\mathbf{S}}

%-------------------------------------------------------------------------------
% v^2-f
\newcommand{\vsq}{\avrg{v^2}}
\newcommand{\ff}{f}
\newcommand{\vsqf}{\vsq-\ff}
\newcommand{\kepsvvf}{\keps-\vsqf}
% constants
\newcommand{\Cl}{C_{L}}
\newcommand{\Ct}{C_{T}}

%-------------------------------------------------------------------------------
\newcommand{\tvisc}{\nu_t}
\newcommand{\vvisc}{\tilde\nu}
\newcommand{\vvort}{\tilde S}
\newcommand{\Cbo}{C_{b1}}
\newcommand{\Cb}[1]{C_{b #1}}
\newcommand{\Cw}[1]{C_{w #1}}
\newcommand{\Cnu}[1]{C_{\nu #1}}
\newcommand{\Fnu}[1]{f_{\nu #1}}

